D-critical locus structure on the Hilbert schemes of some local toric Calabi-Yau threefolds

The notion of a d-critical locus is an ingredient in the definition of motivic Donaldson-Thomas invariants by [BJM19]. In this paper we show that there is a d-critical locus structure on the Hilbert scheme of dimension zero subschemes on some local toric Calabi-Yau 3-folds. We also show that using this d-critical locus structure and a choice of orientation data, the resulting motivic invariants agree with the definition given by the previous work of [BBS13].

==> mrl.tex <==
%% *** Biblography style for Mathematical Research Letters ***

ENTRY
{ address
	author
	booktitle
	chapter
	edition
	editor
	eid
	howpublished
	institution
	isbn
	journal
	key
	month
	note
	number
	organization
	pages
	publisher
	school
	series
	title
	type
	volume
	year
}
{}
{ label }
INTEGERS { output.state before.all mid.sentence after.sentence after.block }
FUNCTION {init.state.consts}
{ #0 'before.all :=
	#1 'mid.sentence :=
	#2 'after.sentence :=
	#3 'after.block :=
}
STRINGS { s t}
FUNCTION {output.nonnull}
{ 's :=
	output.state mid.sentence =
	{ ", " * write$ }
	{ output.state after.block =
		{ add.period$ write$
			newline$
			"\newblock " write$
		}
		{ output.state before.all =
			'write$
			{ add.period$ " " * write$ }
			if$
		}
		if$
		mid.sentence 'output.state :=
	}
	if$
	s
}
FUNCTION {output}
{ duplicate$ empty$
	'pop$
	'output.nonnull
	if$
}
FUNCTION {output.check}
{ 't :=
	duplicate$ empty$
	{ pop$ "empty " t * " in " * cite$ * warning$ }
	'output.nonnull
	if$
}
FUNCTION {fin.entry}
{ add.period$
	write$
	newline$
}

FUNCTION {new.block}
{ output.state before.all =
	'skip$
	{ after.block 'output.state := }
	if$
}
FUNCTION {new.sentence}
{ output.state after.block =
	'skip$
	{ output.state before.all =
		'skip$
		{ after.sentence 'output.state := }
		if$
	}
	if$
}
FUNCTION {add.blank}
{  " " * before.all 'output.state :=
}

FUNCTION {date.block}
{
	skip$
}

FUNCTION {not}
{   { #0 }
	{ #1 }
	if$
}
FUNCTION {and}
{   'skip$
	{ pop$ #0 }
	if$
}
FUNCTION {or}
{   { pop$ #1 }
	'skip$
	if$
}
FUNCTION {new.block.checka}
{ empty$
	'skip$
	'new.block
	if$
}
FUNCTION {new.block.checkb}
{ empty$
	swap$ empty$
	and
	'skip$
	'new.block
	if$
}
FUNCTION {new.sentence.checka}
{ empty$
	'skip$
	'new.sentence
	if$
}
FUNCTION {new.sentence.checkb}
{ empty$
	swap$ empty$
	and
	'skip$
	'new.sentence
	if$
}
FUNCTION {field.or.null} % 1 on the top of the stack if null 
{ duplicate$ empty$
	{ pop$ "" }
	'skip$
	if$
}
FUNCTION {emphasize}
{ duplicate$ empty$
	{ pop$ "" }
	{ "\emph{" swap$ * "}" * }
	if$
}
FUNCTION {bolden}
{ duplicate$ empty$
	{ pop$ "" }
	{ "\textbf{" swap$ * "}" * }
	if$
}
FUNCTION {tie.or.space.prefix}
{ duplicate$ text.length$ #3 <
	{ "~" }
	{ " " }
	if$
	swap$
}

FUNCTION {capitalize}
{ "u" change.case$ "t" change.case$ }

FUNCTION {space.word}
{ " " swap$ * " " * }
% Here are the language-specific definitions for explicit words.
% Each function has a name bbl.xxx where xxx is the English word.
% The language selected here is ENGLISH
FUNCTION {bbl.and}
{ "and"}

FUNCTION {bbl.etal}
{ "et~al." }

FUNCTION {bbl.editors}
{ "editors" }

FUNCTION {bbl.editor}
{ "editor" }

FUNCTION {bbl.edby}
{ "edited by" }

FUNCTION {bbl.edition}
{ "edition" }

FUNCTION {bbl.volume}
{ "Vol." }

FUNCTION {bbl.of}
{ "of" }

FUNCTION {bbl.number}
{ "number" }

FUNCTION {bbl.nr}
{ "no." }

FUNCTION {bbl.in}
{ "in" }

FUNCTION {bbl.pages}
{ "" }

FUNCTION {bbl.page}
{ "" }

FUNCTION {bbl.chapter}
{ "chapter" }

FUNCTION {bbl.techrep}
{ "Technical Report" }

FUNCTION {bbl.mthesis}
{ "Master's thesis" }

FUNCTION {bbl.phdthesis}
{ "Ph.D. thesis" }

MACRO {jan} {"January"}
MACRO {feb} {"February"}
MACRO {mar} {"March"}
MACRO {apr} {"April"}
MACRO {may} {"May"}
MACRO {jun} {"June"}
MACRO {jul} {"July"}
MACRO {aug} {"August"}
MACRO {sep} {"September"}
MACRO {oct} {"October"}
MACRO {nov} {"November"}
MACRO {dec} {"December"}

FUNCTION {bibinfo.check}
{ swap$ 
	duplicate$ missing$ 
	{
		pop$ pop$
		""
	}
	{ duplicate$ empty$
		{
			swap$ pop$
		}
		{ swap$
			pop$
		}
		if$
	}
	if$
}
FUNCTION {bibinfo.warn}
{ swap$
	duplicate$ missing$
	{
		swap$ "missing " swap$ * " in " * cite$ * warning$ pop$
		""
	}
	{ duplicate$ empty$
		{
			swap$ "empty " swap$ * " in " * cite$ * warning$
		}
		{ swap$
			pop$
		}
		if$
	}
	if$
}
STRINGS  { bibinfo}
INTEGERS { nameptr namesleft numnames }

FUNCTION {format.names}
{ 'bibinfo :=
	duplicate$ empty$ 'skip$ {
		's :=
		"" 't :=
		#1 'nameptr :=
		s num.names$ 'numnames :=
		numnames 'namesleft :=
		{ namesleft #0 > }
		{ s nameptr
			"{f.~}{vv~}{ll}{, jj}"
			format.name$
			bibinfo bibinfo.check
			't :=
			nameptr #1 >
			{
				namesleft #1 >
				{ ", " * t * }
				{
					s nameptr "{ll}" format.name$ duplicate$ "others" =
					{ 't := }
					{ pop$ }
					if$
					numnames #2 >
					{ "," * }
					'skip$
					if$
					t "others" =
					{
						" " * bbl.etal *
					}
					{
						bbl.and
						space.word * t *
					}
					if$
				}
				if$
			}
			't
			if$
			nameptr #1 + 'nameptr :=
			namesleft #1 - 'namesleft :=
		}
		while$
	} if$
}
FUNCTION {format.names.ed}
{
	format.names
}
FUNCTION {format.authors}
{ author "author" format.names
}
FUNCTION {get.bbl.editor}
{ editor num.names$ #1 > 'bbl.editors 'bbl.editor if$ }

FUNCTION {format.editors}
{ editor "editor" format.names duplicate$ empty$ 'skip$
	{
		"," *
		" " *
		get.bbl.editor
		*
	}
	if$
}
FUNCTION {format.isbn}
{ isbn "isbn" bibinfo.check
	duplicate$ empty$ 'skip$
	{
		"ISBN " swap$ *
	}
	if$
}

FUNCTION {format.note}
{
	note empty$
	{ "" }
	{ note #1 #1 substring$
		duplicate$ "{" =
			'skip$
			{ output.state mid.sentence =
				{ "l" }
				{ "u" }
				if$
				change.case$
			}
			if$
			note #2 global.max$ substring$ * "note" bibinfo.check
		}
		if$
	}
	
	FUNCTION {format.title}
	{ title
		"title" bibinfo.check
		duplicate$ empty$ 'skip$
		{
			emphasize
		}
		if$
	}
	FUNCTION {output.bibitem}
	{ newline$
		"\bibitem{" write$
			cite$ write$
			"}" write$
		newline$
		""
		before.all 'output.state :=
	}
	
	FUNCTION {n.dashify}
	{
		't :=
		""
		{ t empty$ not }
		{ t #1 #1 substring$ "-" =
			{ t #1 #2 substring$ "--" = not
				{ "--" *
					t #2 global.max$ substring$ 't :=
				}
				{   { t #1 #1 substring$ "-" = }
					{ "-" *
						t #2 global.max$ substring$ 't :=
					}
					while$
				}
				if$
			}
			{ t #1 #1 substring$ *
				t #2 global.max$ substring$ 't :=
			}
			if$
		}
		while$
	}
	
	FUNCTION {word.in}
	{ bbl.in
		" " * }
	
	FUNCTION {format.date}
	{
		""
		duplicate$ empty$
		year  "year"  bibinfo.check duplicate$ empty$
		{ swap$ 'skip$
			{ "there's a month but no year in " cite$ * warning$ }
			if$
			*
		}
		{ swap$ 'skip$
			{
				swap$
				" " * swap$
			}
			if$
			*
		}
		if$
		duplicate$ empty$
		'skip$
		{
			before.all 'output.state :=
			" (" swap$ * ")" *
		}
		if$
	}
	FUNCTION{format.year}
	{ year "year" bibinfo.check duplicate$ empty$
		{  "empty year in " cite$ *
			warning$
		}
		{
			" (" swap$ * ")" *
		}
		if$
	}
	FUNCTION {format.btitle}
	{ title "title" bibinfo.check
		duplicate$ empty$ 'skip$
		{
		}
		if$
	}
	FUNCTION {either.or.check}
	{ empty$
		'pop$
		{ "can't use both " swap$ * " fields in " * cite$ * warning$ }
		if$
	}
	FUNCTION {format.bvolume}
	{ volume empty$
		{ "" }
		{ bbl.volume volume tie.or.space.prefix
			"volume" bibinfo.check * *
			series "series" bibinfo.check
			duplicate$ empty$ 'pop$
			{ swap$ bbl.of space.word * swap$
				emphasize * }
			if$
			"volume and number" number either.or.check
		}
		if$
	}
	FUNCTION {format.number.series}
	{ volume empty$
		{ number empty$
			{ series field.or.null }
			{ series empty$
				{ number "number" bibinfo.check }
				{ output.state mid.sentence =
					{ bbl.number }
					{ bbl.number capitalize }
					if$
					number tie.or.space.prefix "number" bibinfo.check * *
					bbl.in space.word *
					series "series" bibinfo.check *
				}
				if$
			}
			if$
		}
		{ "" }
		if$
	}
	
	FUNCTION {format.edition}
	{ edition duplicate$ empty$ 'skip$
		{
			output.state mid.sentence =
			{ "l" }
			{ "t" }
			if$ change.case$
			"edition" bibinfo.check
			" " * bbl.edition *
		}
		if$
	}
	INTEGERS { multiresult }
	FUNCTION {multi.page.check}
	{ 't :=
		#0 'multiresult :=
		{ multiresult not
			t empty$ not
			and
		}
		{ t #1 #1 substring$
			duplicate$ "-" =
			swap$ duplicate$ "," =
			swap$ "+" =
			or or
			{ #1 'multiresult := }
			{ t #2 global.max$ substring$ 't := }
			if$
		}
		while$
		multiresult
	}
	FUNCTION {format.pages}
	{ pages duplicate$ empty$ 'skip$
		{ duplicate$ multi.page.check
			{
				n.dashify
			}
			{
			}
			if$
			"pages" bibinfo.check
		}
		if$
	}
	FUNCTION {format.journal.pages}
	{ pages duplicate$ empty$ {pop$ "\hskip -.1cm" *}
		{ swap$ duplicate$ empty$
			{ pop$ pop$ format.pages }
			{
				" " *
				swap$
				n.dashify
				"pages" bibinfo.check
				*
			}
			if$
		}
		if$
	}
	FUNCTION {format.journal.eid}
	{ eid "eid" bibinfo.check
		duplicate$ empty$ 'pop$
		{ swap$ duplicate$ empty$ 'skip$
			{
				" " *
			}
			if$
			swap$ *
		}
		if$
	}
	FUNCTION {format.vol.num.pages}
	{ volume field.or.null
		duplicate$ empty$ 'skip$
		{
			"volume" bibinfo.check
		}
		if$
		bolden
		format.year *
		number "number" bibinfo.check duplicate$ empty$ 'skip$
		{
			swap$ duplicate$ empty$
			{ "there's a number but no volume in " cite$ * warning$ }
			'skip$
			if$
			swap$
			", " bbl.nr * number tie.or.space.prefix pop$ *
			swap$ * ", " *
		}
		if$ *
		eid empty$
		{ format.journal.pages }
		{ format.journal.eid }
		if$
	}
	
	FUNCTION {format.chapter.pages}
	{ chapter empty$
		'format.pages
		{ type empty$
			{ bbl.chapter }
			{ type "l" change.case$
				"type" bibinfo.check
			}
			if$
			chapter tie.or.space.prefix
			"chapter" bibinfo.check
			* *
			pages empty$
			'skip$
			{ ", " * format.pages * }
			if$
		}
		if$
	}
	
	FUNCTION {format.booktitle}
	{
		booktitle "booktitle" bibinfo.check
	}
	FUNCTION {format.in.ed.booktitle}
	{ format.booktitle duplicate$ empty$ 'skip$
		{
			editor "editor" format.names.ed duplicate$ empty$ 'pop$
			{
				"," *
				" " *
				get.bbl.editor
				", " *
				* swap$
				* }
			if$
			word.in swap$ *
		}
		if$
	}
	FUNCTION {empty.misc.check}
	{ author empty$ title empty$ howpublished empty$
		month empty$ year empty$ note empty$
		and and and and and
		key empty$ not and
		{ "all relevant fields are empty in " cite$ * warning$ }
		'skip$
		if$
	}
	FUNCTION {format.thesis.type}
	{ type duplicate$ empty$
		'pop$
		{ swap$ pop$
			"t" change.case$ "type" bibinfo.check
		}
		if$
	}
	FUNCTION {format.tr.number}
	{ number "number" bibinfo.check
		type duplicate$ empty$
		{ pop$ bbl.techrep }
		'skip$
		if$
		"type" bibinfo.check
		swap$ duplicate$ empty$
		{ pop$ "t" change.case$ }
		{ tie.or.space.prefix * * }
		if$
	}
	FUNCTION {format.article.crossref}
	{
		key duplicate$ empty$
		{ pop$
			journal duplicate$ empty$
			{ "need key or journal for " cite$ * " to crossref " * crossref * warning$ }
			{ "journal" bibinfo.check emphasize word.in swap$ * }
			if$
		}
		{ word.in swap$ * " " *}
		if$
		" \cite{" * crossref * "}" *
	}
	FUNCTION {format.crossref.editor}
	{ editor #1 "{vv~}{ll}" format.name$
		"editor" bibinfo.check
		editor num.names$ duplicate$
		#2 >
		{ pop$
			"editor" bibinfo.check
			" " * bbl.etal
			*
		}
		{ #2 <
			'skip$
			{ editor #2 "{ff }{vv }{ll}{ jj}" format.name$ "others" =
				{
					"editor" bibinfo.check
					" " * bbl.etal
					*
				}
				{
					bbl.and space.word
					* editor #2 "{vv~}{ll}" format.name$
					"editor" bibinfo.check
					*
				}
				if$
			}
			if$
		}
		if$
	}
	FUNCTION {format.book.crossref}
	{ volume duplicate$ empty$
		{ "empty volume in " cite$ * "'s crossref of " * crossref * warning$
			pop$ word.in
		}
		{ bbl.volume
			swap$ tie.or.space.prefix "volume" bibinfo.check * * bbl.of space.word *
		}
		if$
		editor empty$
		editor field.or.null author field.or.null =
		or
		{ key empty$
			{ series empty$
				{ "need editor, key, or series for " cite$ * " to crossref " *
					crossref * warning$
					"" *
				}
				{ series emphasize * }
				if$
			}
			{ key * }
			if$
		}
		{ format.crossref.editor * }
		if$
		" \cite{" * crossref * "}" *
	}
	FUNCTION {format.incoll.inproc.crossref}
	{
		editor empty$
		editor field.or.null author field.or.null =
		or
		{ key empty$
			{ format.booktitle duplicate$ empty$
				{ "need editor, key, or booktitle for " cite$ * " to crossref " *
					crossref * warning$
				}
				{ word.in swap$ * }
				if$
			}
			{ word.in key * " " *}
			if$
		}
		{ word.in format.crossref.editor * " " *}
		if$
		" \cite{" * crossref * "}" *
	}
	FUNCTION {format.org.or.pub}
	{ 't :=
		""
		address empty$ t empty$ and
		'skip$
		{
			t empty$
			{ address "address" bibinfo.check *
			}
			{ t *
				address empty$
				'skip$
				{ ", " * address "address" bibinfo.check * }
				if$
			}
			if$
		}
		if$
	}
	FUNCTION {format.publisher.address}
	{ publisher "publisher" bibinfo.warn format.org.or.pub
	}
	
	FUNCTION {format.organization.address}
	{ organization "organization" bibinfo.check format.org.or.pub
	}
	
	STRINGS {oldname}
	
	FUNCTION {name.or.dash}
	{ 's :=
		oldname empty$
		{ s 'oldname := s }
		{ s oldname =
			{ "---{}---{}---" }
			{ s 'oldname := s }
			if$
		}
		if$
	}
	
	FUNCTION {article}
	{ output.bibitem
		format.authors "author" output.check
		name.or.dash
		format.title "title" output.check
		crossref missing$
		{
			journal
			"journal" bibinfo.check
			"journal" output.check
			add.blank
			format.vol.num.pages output
		}
		{ format.article.crossref output.nonnull
			format.pages output
		}
		if$
		new.sentence
		format.note output
		fin.entry
	}
	FUNCTION {book}
	{ output.bibitem
		author empty$
		{ format.editors "author and editor" output.check
			name.or.dash
		}
		{ format.authors output.nonnull
			name.or.dash
			crossref missing$
			{ "author and editor" editor either.or.check }
			'skip$
			if$
		}
		if$
		format.btitle "title" output.check
		crossref missing$
		{ format.bvolume output
			format.number.series output
			format.publisher.address output
		}
		{
			format.book.crossref output.nonnull
		}
		if$
		format.edition output
		format.date "year" output.check
		format.isbn output
		new.sentence
		format.note output
		fin.entry
	}
	FUNCTION {booklet}
	{ output.bibitem
		format.authors output
		name.or.dash
		format.title "title" output.check
		howpublished "howpublished" bibinfo.check output
		address "address" bibinfo.check output
		format.date output
		format.isbn output
		new.sentence
		format.note output
		fin.entry
	}
	
	FUNCTION {inbook}
	{ output.bibitem
		author empty$
		{ format.editors "author and editor" output.check
			name.or.dash
		}
		{ format.authors output.nonnull
			name.or.dash
			crossref missing$
			{ "author and editor" editor either.or.check }
			'skip$
			if$
		}
		if$
		format.btitle "title" output.check
		crossref missing$
		{
			format.bvolume output
			format.chapter.pages "chapter and pages" output.check
			format.number.series output
			format.publisher.address output
		}
		{
			format.chapter.pages "chapter and pages" output.check
			format.book.crossref output.nonnull
		}
		if$
		format.edition output
		format.date "year" output.check
		crossref missing$
		{ format.isbn output }
		'skip$
		if$
		new.sentence
		format.note output
		fin.entry
	}
	
	FUNCTION {incollection}
	{ output.bibitem
		format.authors "author" output.check
		name.or.dash
		format.title "title" output.check
		crossref missing$
		{ format.in.ed.booktitle "booktitle" output.check
			format.bvolume output
			format.number.series output
			format.chapter.pages output
			format.publisher.address output
			format.edition output
			format.date "year" output.check
			format.isbn output
		}
		{ format.incoll.inproc.crossref output.nonnull
			format.chapter.pages output
		}
		if$
		new.sentence
		format.note output
		fin.entry
	}
	FUNCTION {inproceedings}
	{ output.bibitem
		format.authors "author" output.check
		name.or.dash
		format.title "title" output.check
		crossref missing$
		{ format.in.ed.booktitle "booktitle" output.check
			format.bvolume output
			format.number.series output
			format.pages output
			publisher empty$
			{ format.organization.address output }
			{ organization "organization" bibinfo.check output
				format.publisher.address output
			}
			if$
			format.date "year" output.check
			format.isbn output
		}
		{ format.incoll.inproc.crossref output.nonnull
			format.pages output
		}
		if$
		new.sentence
		format.note output
		fin.entry
	}
	FUNCTION {conference} { inproceedings }
	FUNCTION {manual}
	{ output.bibitem
		author empty$
		{ organization "organization" bibinfo.check
			duplicate$ empty$ 'pop$
			{ output
				address "address" bibinfo.check output
			}
			if$
		}
		{ format.authors output.nonnull }
		if$
		name.or.dash
		format.btitle "title" output.check
		author empty$
		{ organization empty$
			{
				address "address" bibinfo.check output
			}
			'skip$
			if$
		}
		{
			organization "organization" bibinfo.check output
			address "address" bibinfo.check output
		}
		if$
		format.edition output
		format.date output
		new.sentence
		format.note output
		fin.entry
	}
	
	FUNCTION {mastersthesis}
	{ output.bibitem
		format.authors "author" output.check
		name.or.dash
		format.btitle
		"title" output.check
		bbl.mthesis format.thesis.type output.nonnull
		school "school" bibinfo.warn output
		address "address" bibinfo.check output
		format.date "year" output.check
		new.sentence
		format.note output
		fin.entry
	}
	
	FUNCTION {misc}
	{ output.bibitem
		format.authors output
		name.or.dash
		format.title output
		howpublished "howpublished" bibinfo.check output
		format.date output
		new.sentence
		format.note output
		fin.entry
		empty.misc.check
	}
	FUNCTION {phdthesis}
	{ output.bibitem
		format.authors "author" output.check
		name.or.dash
		format.btitle
		"title" output.check
		bbl.phdthesis format.thesis.type output.nonnull
		school "school" bibinfo.warn output
		address "address" bibinfo.check output
		format.date "year" output.check
		new.sentence
		format.note output
		fin.entry
	}
	
	FUNCTION {proceedings}
	{ output.bibitem
		editor empty$
		{ organization "organization" bibinfo.check output
		}
		{ format.editors output.nonnull }
		if$
		name.or.dash
		format.btitle "title" output.check
		format.bvolume output
		format.number.series output
		editor empty$
		{ publisher empty$
			'skip$
			{
				format.publisher.address output
			}
			if$
		}
		{ publisher empty$
			{
				format.organization.address output }
			{
				organization "organization" bibinfo.check output
				format.publisher.address output
			}
			if$
		}
		if$
		format.date "year" output.check
		format.isbn output
		new.sentence
		format.note output
		fin.entry
	}
	
	FUNCTION {techreport}
	{ output.bibitem
		format.authors "author" output.check
		name.or.dash
		format.title
		"title" output.check
		format.tr.number output.nonnull
		institution "institution" bibinfo.warn output
		address "address" bibinfo.check output
		format.date "year" output.check
		new.sentence
		format.note output
		fin.entry
	}
	
	FUNCTION {unpublished}
	{ output.bibitem
		format.authors "author" output.check
		name.or.dash
		format.title "title" output.check
		format.date output
		new.sentence
		format.note "note" output.check
		fin.entry
	}
	
	FUNCTION {default.type} { misc }
	READ
	FUNCTION {sortify}
	{ purify$
		"l" change.case$
	}
	INTEGERS { len }
	FUNCTION {chop.word}
	{ 's :=
		'len :=
		s #1 len substring$ =
		{ s len #1 + global.max$ substring$ }
		's
		if$
	}
	FUNCTION {sort.format.names}
	{ 's :=
		#1 'nameptr :=
		""
		s num.names$ 'numnames :=
		numnames 'namesleft :=
		{ namesleft #0 > }
		{ s nameptr
			"{vv{ } }{ll{ }}{  f{ }}{  jj{ }}"
			format.name$ 't :=
			nameptr #1 >
			{
				"   "  *
				namesleft #1 = t "others" = and
				{ "zzzzz" * }
				{ t sortify * }
				if$
			}
			{ t sortify * }
			if$
			nameptr #1 + 'nameptr :=
			namesleft #1 - 'namesleft :=
		}
		while$
	}
	
	FUNCTION {sort.format.title}
	{ 't :=
		"A " #2
		"An " #3
		"The " #4 t chop.word
		chop.word
		chop.word
		sortify
		#1 global.max$ substring$
	}
	FUNCTION {author.sort}
	{ author empty$
		{ key empty$
			{ "to sort, need author or key in " cite$ * warning$
				""
			}
			{ key sortify }
			if$
		}
		{ author sort.format.names }
		if$
	}
	FUNCTION {author.editor.sort}
	{ author empty$
		{ editor empty$
			{ key empty$
				{ "to sort, need author, editor, or key in " cite$ * warning$
					""
				}
				{ key sortify }
				if$
			}
			{ editor sort.format.names }
			if$
		}
		{ author sort.format.names }
		if$
	}
	FUNCTION {author.organization.sort}
	{ author empty$
		{ organization empty$
			{ key empty$
				{ "to sort, need author, organization, or key in " cite$ * warning$
					""
				}
				{ key sortify }
				if$
			}
			{ "The " #4 organization chop.word sortify }
			if$
		}
		{ author sort.format.names }
		if$
	}
	FUNCTION {editor.organization.sort}
	{ editor empty$
		{ organization empty$
			{ key empty$
				{ "to sort, need editor, organization, or key in " cite$ * warning$
					""
				}
				{ key sortify }
				if$
			}
			{ "The " #4 organization chop.word sortify }
			if$
		}
		{ editor sort.format.names }
		if$
	}
	FUNCTION {presort}
	{ type$ "book" =
		type$ "inbook" =
		or
		'author.editor.sort
		{ type$ "proceedings" =
			'editor.organization.sort
			{ type$ "manual" =
				'author.organization.sort
				'author.sort
				if$
			}
			if$
		}
		if$
		"    "
		*
		year field.or.null sortify
		*
		"    "
		*
		title field.or.null
		sort.format.title
		*
		#1 entry.max$ substring$
		'sort.key$ :=
	}
	ITERATE {presort}
	SORT
	STRINGS { longest.label }
	INTEGERS { number.label longest.label.width }
	FUNCTION {initialize.longest.label}
	{ "" 'longest.label :=
		#1 'number.label :=
		#0 'longest.label.width :=
	}
	FUNCTION {longest.label.pass}
	{ number.label int.to.str$ 'label :=
		number.label #1 + 'number.label :=
		label width$ longest.label.width >
		{ label 'longest.label :=
			label width$ 'longest.label.width :=
		}
		'skip$
		if$
	}
	EXECUTE {initialize.longest.label}
	ITERATE {longest.label.pass}
	FUNCTION {begin.bib}
	{ preamble$ empty$
		'skip$
		{ preamble$ write$ newline$ }
		if$
		"\begin{thebibliography}{"  longest.label  * "}" *
			write$ newline$
		}
		EXECUTE {begin.bib}
		EXECUTE {init.state.consts}
		ITERATE {call.type$}
		FUNCTION {end.bib}
		{ newline$
			"\end{thebibliography}" write$ newline$
	}
	EXECUTE {end.bib}
